Scene Synthesis via Uncertainty-Driven Attribute Synchronization

Developing deep neural networks to generate 3D scenes is a fundamental problem in neural synthesis with immediate applications in architectural CAD, computer graphics, as well as in generating virtual robot training environments. This task is challenging because 3D scenes exhibit diverse patterns, ranging from continuous ones, such as object sizes and the relative poses between pairs of shapes, to discrete patterns, such as occurrence and co-occurrence of objects with symmetrical relationships. This paper introduces a novel neural scene synthesis approach that can capture diverse feature patterns of 3D scenes. Our method combines the strength of both neural network-based and conventional scene synthesis approaches. We use the parametric prior distributions learned from training data, which provide uncertainties of object attributes and relative attributes, to regularize the outputs of feed-forward neural models. Moreover, instead of merely predicting a scene layout, our approach predicts an over-complete set of attributes. This methodology allows us to utilize the underlying consistency constraints among the predicted attributes to prune infeasible predictions. Experimental results show that our approach outperforms existing methods considerably. The generated 3D scenes interpolate the training data faithfully while preserving both continuous and discrete feature patterns.

==> sections/results.tex <==
\section{Results}
\label{sec:result}

In this section, we present an experimental evaluation of the proposed approach. In Section~\ref{subsec:setup}, we describe the experimental setup for datasets and also baseline methods. In Section~\ref{subsec:results}, we demonstrate the results of our approach and compare it with baseline methods. We analyze each components of our approach in Section~\ref{subsec:analysis}.

\subsection{Experimental Setup}
\label{subsec:setup}
%Architecture dataset:
%\begin{itemize}
%    \item 3D-Street-View Dataset (2016): \cite{zamir2016generic}. The dataset contains the 3D models of 7 cities. Each city is stored as a single mesh so it need to be partitioned manually in order to get the individual architecture models. 
%   % Sample images are shown in Figure \ref{fig:dataset_example:eu} and Figure \ref{fig:dataset_example:us}.  
%\end{itemize}
%
%\begin{figure}
%    \centering
%    \includegraphics[width=0.5\textwidth]{figs/dataset_example/eu_data_example.png}
%    \caption{Architectures in Europe}
%    \label{fig:dataset_example:eu}
%\end{figure}
%\begin{figure}
%    \centering
%    \includegraphics[width=0.5\textwidth]{figs/dataset_example/us_data_example.png}
%    \caption{Architectures in US}
%    \label{fig:dataset_example:us}
%\end{figure}
\paragraph{Dataset.}
We perform experimental evaluation mainly on PartNet\cite{mo2019partnet} in this paper. Following the data preparation from Structurenet\cite{mo2019structurenet}, we use three largest categories in our experiments: chairs, tables, cabinets, where each of them contains 4871, 5099, 862 examples. To parameterize the 3D parts, we assume each part belongs to one of $c$ classes and each class contains the maximum number of $N_c$ parts. In our experiment, we set $c = 5$ and $N_c = 12$ for the chair object. 

\paragraph{Baseline approaches.}
There are several existing methods on synthesizing shapes as geometric arrangements of predefined primitives and components. We pick the most competitive methods GRASS~\cite{Li2017GRASS} and S-Net~\cite{mo2019structurenet} as baseline approaches.

\subsection{Experimental Results}
\label{subsec:results}

\begin{table}[]
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c}
       & Chair & Table & Cabinet  & Trashcan & Vase\\
       \hline
       GRASS & - & - & - & - & -  \\
       S - Net  & 0.062 & 0.073 & 0.066  & 0.083 & 0.147\\
       Ours-A & 0.052 & 0.052 & 0.059 & - & -\\
       Ours & - & - & - & - & -\\
    \end{tabular}
    \caption{Reconstruction performance on each shape category. We
compare the reconstruction performance of our method and baseline model on three shape categories.}
    \label{tab:recon}
\end{table}
%\begin{itemize}
%    \item \textbf{StructureNet.} The typical failure cases of StructureNet is shown in Figure. \ref{fig:result:fail_structurenet}. StructureNet will sometimes generate asymmetric parts, duplicated parts and detached parts because it only uses loss function to regularize the relations between parts.
%    \item \textbf{ShapeAssembly.} Failure cases: extra parts, disconnected parts, shift (not global symmetric)
%\end{itemize}
%
%\begin{figure}
%    \centering
%    \includegraphics[width=0.5\textwidth]{figs/result/fail_structurenet.png}
%    \caption{Typical failure cases of StructureNet}
%    \label{fig:result:fail_structurenet}
%\end{figure}

\subsection{Analysis of Our Approach}
\label{subsec:analysis}
\begin{figure*}
\includegraphics[width=1.0\textwidth]{Figures/Absolute_Distribution.png}
\caption{Distributions of absolute primitive parameters. We show distributions of five part parts under distributions of scales in each dimension, rotation axis, rotation angles, and translations along each axis. In each block, we should the distribution of the training data, the distribution of the prediction output, and the distribution of the final output. }
\label{Figure:Absoluate:Prediction}
\end{figure*}

This section presents an analysis on different components of our approach. Our goal is to analyze whether important statistics of the training data, such as the mean and covariance of the different predictions are consistent with those from the training data. For simplicity, we perform our experimental study using the PartNet~\cite{mo2019partnet} benchmark dataset. 

\paragraph{Analysis of absolute parameter predictions.}
We first analyze predictions of absolute parameters from the output of the prediction module. As illustrated in Figure~\ref{Figure:Absoluate:Prediction}, the alignments between the predicted distributions and those of the training data vary across different parts and coordinates. For example, the part scalings are predicted well by the prediction network. So do rotations of part seats and part backs that have dominant part poses. However, distributions of part locations are preserved less well. So do distributions of rotations of chair legs. Such results are expected as absolute parameters do not explicitly enforce the spacial part relations, which are critical for determining part locations. 

\begin{figure}%[h]
\includegraphics[width=1.0\columnwidth]{Figures/Absolute_Covariance.png}
\caption{Covariance matrix among the absolute primitive parameters. }
\label{Figure:Absolute:Covariance}
\end{figure}

Figure~\ref{Figure:Absolute:Covariance} shows the covariance matrix among different part coordinates. We can see that the predictions of correlations of part coordinates across different parts are far less accurate than those of the same parts. This indicates that using absolute primitive parts alone do not provide accurate synthesized geometry arrangements. 

\paragraph{Analysis of relative parameter predictions.}
Figure~\ref{Figure:Relative:Prediction} illustrates the distributions of three relative primitive parameters, i.e., the one derived from the training data, the one derived from absolute primitive parameters, and the predicted relative parameters. We can see that one part pairs that exhibit strong correlations, e.g., between chair seat and chair leg and between chair seat and parts on chair back, the predicted relative parameters are generally more accurate than those derived from absolute parameters. For example, the KL divergence of the relative distribution in part locations between chair leg and chair seat is improved from xxx to xxx. These statistics justify our design goal of explicitly predicting relative parameters of correlated primitives. On the other hand, for part pairs that do not exhibit strong correlations, e.g., between chair back and chair legs, the accuracy of the direct prediction is comparable to that derived from the absolute parameters. Our approach addresses this issue by using a robust norm to prune out inaccurate relative predictions.


\begin{figure*}
\includegraphics[width=1.0\textwidth]{Figures/Relative_Distribution.png}
\caption{Distributions of relative primitive parameters. We show distributions of four part pairs under distributions of scales in each dimension, relative rotation axis, relative rotation angles, and relative translations along each axis. In each block, we should the distribution of the training data, the distribution derived from absolute primitive parameters, and the distribution of the predicted relative parameters. }
\label{Figure:Relative:Prediction}
\end{figure*}

\paragraph{Analysis of the synchronization module.}
Figure~\ref{Figure:Absoluate:Prediction} show that distributions of the absolute parameters after synchronization align much better with those from the training data than the direct predictions. For example, poses of chair legs and locations of chair back/seat/legs all result in considerable performance gains from the direction predictions of absolute parameters. For example, the mean KL divergence between distributions of chair parts are improved from xxx (absolute) to xxx (relative). In addition, Figure~\ref{Figure:Absolute:Covariance} show that correlations among different chair parts are significantly improved using the synchronization module. The relative absolute differences between predictions of covaraince matrices are improved from 0.xxx to 0.xxx. Such improvements mainly come from automatically extracting and enforcing accurate predictions of relative parameters. 

\begin{table}[t]
\centering
\small
\begin{tabular}{c|c|c|c|c|c|c}
 & chair & xxxxx & xxxxx & xxxxx & xxxxx & xxxxx\\ \hline
Pred-P & & & & & & \\
Pred-R & & & & & & \\ \hline
Reca-P & & & & & & \\
Pred-R & & & & & & 
\end{tabular}
\vspace{0.0in}
\caption{}
\label{Table:Precision:Recall}
\end{table}

\paragraph{Analysis of the existence indicator variable.}
Finally, we analyze the precision and recall of the existence indicator variable. Table~\ref{Table:Precision:Recall} collect precision/recall of the part existence vector in each category of PartNet. We can see that the final existence prediction leads to performance gains in both precision and recall. In other words, aggregating the consistency scores between absolute parameters and relative parameters provide useful signals to determine primitive indicators. 

